Multi-Codec DASH Dataset

The number of bandwidth-hungry applications and services is constantly growing. HTTP adaptive streaming of audio-visual content accounts for the majority of today's internet traffic. Although the internet bandwidth increases also constantly, audio-visual compression technology is inevitable and we are currently facing the challenge to be confronted with multiple video codecs. This paper proposes a multi-codec DASH dataset comprising AVC, HEVC, VP9, and AV1 in order to enable interoperability testing and streaming experiments for the efficient usage of these codecs under various conditions. We adopt state of the art encoding and packaging options and also provide basic quality metrics along with the DASH segments. Additionally, we briefly introduce a multi-codec DASH scheme and possible usage scenarios. Finally, we provide a preliminary evaluation of the encoding efficiency in the context of HTTP adaptive streaming services and applications.

==> 0_workplan.tex <==
\section{Workplan}

\begin{itemize}
\item Introduction --- CT (Almost DONE)
\item Related work --- CT (DONE)
\item Methodology and Dataset Description: how did we select the sequences and why; encoding parameters; MPD; etc. (basically from ICIP paper) --- AZ, CF
\item Usage/research challenges: for what and how the dataset could be used; player adaptation logic; bandwidth/network allocation; ... --- AZ, CT
\item Metrics and evaluation: PSNR, SSIM, etc. --- AZ
\item Conclusions: currently only a limited set of sequences is available which can be played with firefox nightly builds but we will extend the dataset once AV1 is finalized (code freeze) which is going to happen soon; also it take long to encode --- CT
\item add a new blog post to \url{http://dash.itec.aau.at} --- CT
\item add dataset to \url{http://dash.itec.aau.at} --- AZ
\end{itemize}

